From Legal Contracts to Legal Calculi: the code-driven normativity

Using dedicated software to represent or enact legislation or regulation has the advantage of solving the inherent ambiguity of legal texts and enabling the automation of compliance with legal norms. On the other hand, the so-called code-driven normativity is less flexible than the legal provisions it claims to implement, and transforms the nature of legal protection, potentially reducing the capability of individual human beings to invoke legal remedies. In this article we focus on software-based legal contracts; we illustrate the design of a legal calculus whose primitives allow a direct formalisation of contracts' normative elements (i.e., permissions, prohibitions, obligations, asset transfer, judicial enforcement and openness to the external context). We show that interpreting legal contracts as interaction protocols between (untrusted) parties enables the generalisation of formal methods and tools for concurrent systems to the legal setting

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{V. Castiglioni and C. A. Mezzina (Eds): Combined Workshop on \\ Expressiveness in Concurrency and Structural Operational Semantics 2022 \\ (EXPRESS/SOS 2022).\\
EPTCS 368, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.368.2}{10.4204/EPTCS.368.2}}
\pdfoutput=1

